Who is in Charge here? Understanding How Runtime Configuration Affects Software along with Variables&Constants

Runtime misconfiguration can lead to software performance degradation and even cause failure. Developers typically perform sanity checks during the configuration parsing stage to prevent invalid parameter values. However, we discovered that even valid values that pass these checks can also lead to unexpected severe consequences. Our study reveals the underlying reason: the value of runtime configuration parameters may interact with other constants and variables when propagated and used, altering its original effect on software behavior. Consequently, parameter values may no longer be valid when encountering complex runtime environments and workloads. Therefore, it is extremely challenging for users to properly configure the software before it starts running. This paper presents the first comprehensive and in-depth study (to the best of our knowledge) on how configuration affects software at runtime through the interaction with constants, and variables (PCV Interaction). Parameter values represent user intentions, constants embody developer knowledge, and variables are typically defined by the runtime environment and workload. This interaction essentially illustrates how different roles jointly determine software behavior. In this regard, we studied 705 configuration parameters from 10 large-scale software systems. We reveal that a large portion of configuration parameters interact with constants/variables after parsing. We analyzed the interaction patterns and their effects on software runtime behavior. Furthermore, we highlighted the risks of PCV interaction and identified potential issues behind specific interaction patterns. Our findings expose the "double edge" of PCV interaction, providing new insights and motivating the development of new automated techniques to help users configure software appropriately and assist developers in designing better configurations.

==> 1-finding.tex <==
\begin{table*}
\caption{Summary of our findings on PCV Interactions.}
\vspace{-5pt}
\label{tab: summary of findings}

\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|p{17.676cm}|}
\hline
\rowcolor{VeryLightGray}\textbf{Configuration itself can not rule the world, needing help from other constants and variables. (\S \ref{section: PCV Pattern})}\\
\hline
\textbf{Finding 1: Only one third (33.6\%\Space{, 237 / 70}) of parameters can independently affect software behavior by propagating and using its value faithfully.} The rest of the parameters will interact with constants or variables.\\
\hline
\end{tabular*}
\\[0.1cm]

\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|p{17.676cm}|}
\hline
\rowcolor{VeryLightGray}\textbf{PCV interaction can control software behavior, greatly impacting software performance and reliability. (\S \ref{section: Interaction Effect})}\\
\hline
\textbf{Finding 2: PCV interactions can have a great impact on software performance (\Space{237 / 616 = }38.5\%) and reliability (\Space{257 / 616 = }41.7\%)}. Others are usually the implementation of logical functionalities.\\
\hline
\textbf{Finding 3: P\&C interactions are primarily (81.5\%\Space{, 172/211}) used for misconfiguration prevention.} A good constant used as a checker should incorporate developer knowledge.\\
%Finding 2: Most \red{(206/259=79.5\%)} of the interactions will have effects on software performance \red{(114/206=55.3\%)} and reliability \red{(92/206=44.7\%)}, others \red{(53/259=20.5\%)} only focus on functional and logical implementation. \\
\hline


\textbf{Finding 4: 66.2\%\Space{ (260/393)} of P\&V interactions are used for workload adaption. Among them, 76.2\%\Space{ (198/260)} are to prevent excessive resource utilization.} Which have an important effect on both software performance and reliability.\\
\hline
\end{tabular*}
\\[0.1cm]

\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|p{17.676cm}|}
\hline
\rowcolor{VeryLightGray}\textbf{However, PCV interactions are "under risk". (\S \ref{section: common problems})}\\
\hline
\textbf{Finding 5: More than half (56.5\%\Space{, 349/616}) of the interactions have the potential to cause bad consequences.} This including runtime error (\Space{48/349}13.7\%), performance degradation (\Space{186/349}53.3\%) and unexpected results (\Space{115/349}33.0\%).\\
\hline
\textbf{Finding 6: Existing logs are lack of comprehensive interaction details (or even missing) to assist users in configuration adjustments.} Only a small number of cases (\Space{94/616}15.3\%) explicitly inform users about the interaction information.\\
\hline
\textbf{Finding 7: The software does not provide sufficient support for on-the-fly update of interacted parameters.}
Rare Java software parameters (7/240) support update at runtime.\\
\hline
\end{tabular*}
\\[0.1cm]

\begin{threeparttable}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|p{17.676cm}|}

\hline
\rowcolor{VeryLightGray}\textbf{"Crises" are hidden behind specific interaction patterns. (\S \ref{section: unique problems})}\\
\textbf{Finding 8 (C$\rightarrow$P): The constants used for parameter overwritten in C$\rightarrow$P are not carefully selected and checked.} Among these constants, Lots (\Space{31/56 = }55.4\%) of them differ from the parameter's default value. There are also a few "fake configuration" that the parameter will be mandatory overwritten without checking conditions.\\
\hline
\textbf{Finding 9 (V$\rightarrow$P): During V$\rightarrow$P, developers conditionally modify user-set values to adapt to runtime workload. However, they are not considered comprehensively and thoroughly enough.}
The majority (48/66) of conditional modifications only consider partial scenarios. Some modifications (4/66) only take effect when users do not set parameter values at all.\\
\hline
\textbf{Finding 10 (P$\rightarrow$V): For parameters serving as thresholds in P$\rightarrow$V, they themselves also need appropriate limitations.} Arbitrarily setting their values without thorough consideration of the runtime scenario can lead to severe issues.\\
\hline
\textbf{Finding 11 (P-V): P-V demonstrates the need for tuning switches. A simple switch-off could lose the opportunity for performance optimization even when needed.} \Space{Nearly all }Many of the default values (\Space{14/21=}66.7\%) of parameters used for tuning optimization are false. \\
\hline
\end{tabular*}
\begin{tablenotes}
    \footnotesize
    \item[1] "$\rightarrow$" denotes constraint relationships and "-" denotes equivalent places (detailed definitions in \S \ref{section: PCV Pattern}).
\end{tablenotes}
\end{threeparttable}
\\[0.1cm]
\vspace{-15pt}
\end{table*}

% \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|p{17.45cm}|}
% \hline
% \textbf{Findings on Possible Solutions of Interaction Problems (Section \ref{possible solutions})}\\
% \hline
% Finding 12: In \red{70.4\% (182/259)} of cases, parameter only interact with one constant or variable. In most of \red{(142/182=78.0\%)} of them, the interactions between them are intra-procedural.\\ 
% \hline
% Finding 13: The utilization of thread resources is usually \red{(9/11=81.8\%)} in a loop body and the iterations can be used to adjust the corresponding parameters.\\
% \hline
% \end{tabular*}
% \\[0.1cm]

==> 6-solution.tex <==
\section{Possible solutions of Potential Problems}\label{possible solutions}
In this section, we will discuss potential solutions to the underlying issues of interactions. We delve into the guidance of extracting variables/constants information associated with parameters from the source code, addressing the following key aspects: the complexities inherent in interaction relationships (Section \ref{section: solution complexities}); the possibility of getting workload information for parameters that have no direct interaction relationship with workload-related variables (Section \ref{section: no interaction parameter}).

\subsection{Complexities of Interaction Relationships}\label{section: solution complexities}
We wish to understand the complexities of interaction relationships. Specifically, how many variables/constants are involved in the interactions? 

\begin{center}
    \noindent\fbox{
        \parbox{.97\linewidth}
        {
            \textbf{Finding 12: }In 70.4\% (182/259) of cases, parameters only interact with one constant or variable. In most (142/182=78.0\%) of them, the interactions between them are intra-procedural.
            \\[0.1cm]
            \textbf{Implication:} The interaction relationships are not inherently complex, and workload information associated with parameters can be readily obtained through simple program analysis.
        }
    }
\end{center}

This finding implies that we can solve most of the potential problems by analyzing only one constant or variable. By simply analyzing corresponding variables in these cases, we can get the workload information. 


\subsection{Workload Information without Direct Interaction}\label{section: no interaction parameter}

We can obtain the corresponding workload information by analyzing the variables within the P\&V interaction. But there are still a small portion (16\% to 48\%) of parameters that have no direct interaction relationship. We wish to explore the workload information associated with such parameters so that it is possible to auto-correct them at runtime.

\begin{figure}
\centering
\begin{subfigure}{0.5\textwidth}
    \includegraphics[width=\textwidth]{Figures/yarn thread loop.pdf}
    \caption{Parameters determined the size of thread pool, and the thread resources are utilized within the loop.}
    \label{fig:loopA}
\end{subfigure}
\vspace{5pt}
\hfill
\begin{subfigure}{0.5\textwidth}
    \includegraphics[width=\textwidth]{Figures/hive array.pdf}
    \caption{Parameters determined the length of array, and the array is invoked within the loop.}
    \label{fig:loopB}
\end{subfigure}
\hfill
\vspace{-10pt}
\caption{Resources determined by parameters are usually invoked with the loop.}
\label{fig:loop}
\end{figure}

Some parameters, while not directly interacting with workload-related variables, can be associated with workload information through specific code patterns. Specifically, we find that thread pool objects and array objects (which could also be lists or queues) defined by parameters are frequently utilized within the loop body. Each iteration of the loop typically consumes a unit quantity of resources. Consequently, the length of the loop can be utilized for auto-correcting the parameters.

Figure \ref{fig:loop} illustrates two relevant examples. In Figure \ref{fig:loopA}, \verb|yarn.router.interceptor.user.threadpool-size| determines the number of active threads in the thread pool object (L10). By tracking \verb|executorService|, we find that it executes tasks stored in the list \verb|callables| through \emph{invokeAll()} (L21). The tasks in \verb|callables| are defined from the loop body at L16 to L19, where each iteration adds a task to the \verb|callables| list through the \emph{add()}. To achieve optimal performance, the value of this parameter should not be less than the number of tasks stored in \verb|callables|. Similarly, in Figure \ref{fig:loopB}, the value of \verb|hive.metastore.stats.auto.analyze.worker.count| determines the length of the \verb|workQueue| array. By tracing the propagation and utilization of \verb|workQueue|, we find that it adds work requests \verb|req| by repeatedly calling the \emph{put()} method within the loop (L15). Ideally, the value of the parameter should be greater than or equal to the total number of \verb|req| to ensure that \verb|workQueue| can store all of them.

In both types of examples mentioned above, the length of the loop represents workload information closely associated with parameters. These workload details typically manifest within specific code patterns, namely, the loop body. By tracking specific methods called (e.g., \emph{add()}, \emph{invokeAll()}, and \emph{put()}) by objects defined by parameters, identifying the loops in which they reside, we can extract workload information associated with parameters, providing possibilities for auto-correcting the parameters.

\begin{center}
    \noindent\fbox{
        \parbox{.97\linewidth}
        {
            \textbf{Finding 13:} Most (9/11=81.8\%) of the thread pool and all (6/6=100\%) of the arrays that are determined by parameters will be utilized within the loop body, where the corresponding workload information can be obtained from the length of the loop.
        }
    }
\end{center}

We extracted parameters that determine the definition of thread pools, array lists, and queues from our dataset whose interaction modes are P or P\&V. We further trace the propagation and utilization of these resource objects. The findings revealed that a majority of these resource objects (76.5\%, or 13 out of 17) are employed within loops. Moreover, their associated workload information can be obtained through straightforward static analysis.

\subsection{Good Practice of Developers}
In this section, we explore potential strategies for elastically adjusting configurations based on some good practices among developers. On one hand, there is the approach of fine-tuning user-set parameter values in response to changes in workload. On the other hand, there is the progressive adjustment of parameter values according to the demands of the workload until the user-defined parameter value is reached.

\subsubsection{Elastically setting parameters}

Under normal circumstances, the software employs the values set by users. Throughout the runtime of the software, it is imperative to meticulously monitor the workload and dynamically adjust parameter values in response to fluctuations in the workload.

Figure \ref{fig: Changed based on workload} illustrates an example from MySQL. Under normal circumstances, the variable value \verb|n_pages| used by the software is calculated based on user-set parameter values (L2). During runtime, the software monitors the quantity of UNDO logs in the current tablespace. If the number of UNDO logs increases beyond the default value in the last second (L3), \verb|n_pages| is adjusted to a load-related variable, specifically one-fourth of the old tablespace page count, to adapt to the software's workload conditions (L5).

Developers need to monitor the rate of change in workload. Note that this involves more than simply tracking the quantity of the workload. Based on these variations of workload, adjustments should be made to the parameter values set by the user.

\subsubsection{Elastically changing parameters}
The values set by the user may exceed the demands of the workload. In such cases, we can utilize a smaller value to conserve system resources and gradually increase the number of resources during runtime based on actual requirements. 

\begin{figure}
    \centerline{\includegraphics[width=0.5\textwidth]{Figures/yarn_dynamic_changing.pdf}}
    \caption{Yarn elastically changes the value of parameter according to the demand of workload}
    \label{fig: elastically changing}
\end{figure}

Figure \ref{fig: elastically changing} illustrates an example from Yarn, where \verb|initSize| determines the maximum number of threads in NMClientAsync for processing container management events. Developers initialize the thread pool with a value not exceeding \verb|INITIAL_THREAD_POOL_SIZE| (L4, the value is 10) for resource conservation. During the execution of the \emph{run()}, Yarn assesses the current size of the thread pool (L10) and the number of nodes that need processing (L12). If this surpasses the current thread pool size (L13), the thread pool is increased according to the workload demands, maintaining a certain buffer (L15, L16). \emph{Math.min()} is used to ensure that the thread pool size never exceeds the value set by the user during elastically changing (L11, L13 and L15).

Unlike directly using the parameter values set by the user, here the parameter plays a role similar to a threshold. Developers need to make an initial estimation of the software's startup conditions, quantify the workload during runtime, and flexibly adjust parameters based on the workload until the parameter values align with the user's settings.

==> review.tex <==
Summary:
This paper investigates the interactions between software systems' configuration parameters, constants, and variables. By analyzing 705 configuration parameters across ten large-scale software systems, the authors provide significant insights into how these interactions impact software performance and reliability.

###Strengths:

Addresses a critical aspect of software engineering.
Comprehensive empirical analysis.
Well-structured and clearly presented.

###Weaknesses:

Some technical details need further clarification.
Limited evaluation in certain aspects.

Comments for Authors:

###Rigor
The methodology employed in this study is robust and comprehensive. The manual inspection of 705 configuration parameters across ten software systems showcases a high level of detail and accuracy. However, a few areas could be clarified to enhance the paper's rigor:

Analysis Methodology: The paper should provide more detailed explanations of how the interactions between configuration parameters, constants, and variables were identified and categorized. Clarifying the criteria and methods used for validation would enhance transparency.
Evaluation Metrics: The evaluation is extensive, but including additional metrics such as the impact on software performance and reliability would provide a more holistic view. Comparisons with other similar studies or benchmarks could further strengthen the findings.

###Relevance
The research addresses a crucial aspect of software configuration management, offering insights that are directly applicable to both academic and industrial contexts. The comprehensive analysis of ten different software systems enhances the relevance of the findings, making them valuable for a wide audience involved in software development and maintenance.

###Novelty
The study introduces a novel perspective by focusing on the interactions between configuration parameters, constants, and variables, an area that has not been extensively explored before. This innovative approach uncovers new insights into how configuration impacts software behavior, contributing significantly to the field of software engineering.

###Verifiability and Transparency
The authors make available a GitHub anonymous repository. However, more detailed documentation of the methods and tools used would enhance transparency. For example, providing specific details on the software systems analyzed, the configuration parameters examined, and the tools used for manual inspection would be beneficial.

###Presentation
The paper is well-written and logically structured. Figures and tables are used effectively to support the narrative. Minor improvements in clarity and detail could enhance the overall presentation.


Each pattern in the above CPBug types determines the
oracle of identifying whether there is a CPBug. For example,
with Type-3, we can interpret it as “if a resource allocation
related option is changed from a small value to a larger
value, then we expect the performance to be improved or
otherwise there is a CPBug”. 
Therefore, it is essential to estimate beforehand which CPBug type an option being tested is most likely to be associated with.
